Kvasir-Instrument: Diagnostic and therapeutic tool segmentation dataset in gastrointestinal endoscopy

Gastrointestinal (GI) pathologies are periodically screened, biopsied, and resected using surgical tools. Usually the procedures and the treated or resected areas are not specifically tracked or analysed during or after colonoscopies. Information regarding disease borders, development and amount and size of the resected area get lost. This can lead to poor follow-up and bothersome reassessment difficulties post-treatment. To improve the current standard and also to foster more research on the topic we have released the ``Kvasir-Instrument'' dataset which consists of $590$ annotated frames containing GI procedure tools such as snares, balloons and biopsy forceps, etc. Beside of the images, the dataset includes ground truth masks and bounding boxes and has been verified by two expert GI endoscopists. Additionally, we provide a baseline for the segmentation of the GI tools to promote research and algorithm development. We obtained a dice coefficient score of 0.9158 and a Jaccard index of 0.8578 using a classical U-Net architecture. A similar dice coefficient score was observed for DoubleUNet. The qualitative results showed that the model did not work for the images with specularity and the frames with multiple instruments, while the best result for both methods was observed on all other types of images. Both, qualitative and quantitative results show that the model performs reasonably good, but there is a large potential for further improvements. Benchmarking using the dataset provides an opportunity for researchers to contribute to the field of automatic endoscopic diagnostic and therapeutic tool segmentation for GI endoscopy.

==> takeouts.tex <==
% 
%We aim to develop an accurate and robust method for surgical instrument segmentation from endoscopic images based on computer vision techniques. However, one of the significant problem in the field is lack of publicly available dataset for benchmarking the algorithms and improving the benchmark on the same datasets\cite{jha2020kvasir}. For the Kvasir-instrument dataset, we have used UNet architecture, which is common semantic segmentation based architecture for medical image segmentation tasks. Next, we provide a baseline algorithm that provides and invite multimedia researcher to improve the baseline methods. In this paper, we present our approach for binary instrument segmentation on the endoscopic instrument segmentation dataset. 
